Enhanced Half-Metallicity in Edge-Oxidized Zigzag Graphene Nanoribbons

We present a novel comprehensive first-principles theoretical study of the electronic properties and relative stabilities of edge-oxidized zigzag graphene nanoribbons. The oxidation schemes considered include hydroxyl, carboxyl, ether, and ketone groups. Using screened exchange density functional theory, we show that these oxidized ribbons are more stable than hydrogen-terminated nanoribbons except for the case of the etheric groups. The stable oxidized configurations maintain a spin-polarized ground state with antiferromagnetic ordering localized at the edges, similar to the fully hydrogenated counterparts. More important, edge oxidation is found to lower the onset electric field required to induce half-metallic behavior and extend the overall field range at which the systems remain half-metallic. Once the half-metallic state is reached, further increase of the external electric field intensity produces a rapid decrease in the spin magnetization up to a point where the magnetization is quenched completely. Finally, we find that oxygen containing edge groups have a minor effect on the energy difference between the antiferromagnetic ground state and the above-lying ferromagnetic state.

==> Makefile <==
.SUFFIXES: $(SUFFIXES) .dvi .ps .bib .tex .bbl .pdf

    PAPER_ROOT = OXY-ZZ-GNR

  AIX_PSVIEWER = ghostview
Linux_PSVIEWER = ghostview
SunOS_PSVIEWER = ghostview

INFILES =  OXY-ZZ-GNR.tex \
#	fkt.eps \
#	skw.eps


# PICTURES = 
#
# A very cool hack to "do the right thing":
       PSVIEWER = ${$(OS)_PSVIEWER}
#
#
# standard rules:
#
.dvi.ps:
	touch $*.ps
	/bin/rm $*.ps
	@echo "compiling $*"
	dvips -t a4 -o $*.ps $<

.ps.pdf:
	touch $*.pdf
	/bin/rm $*.pdf
	@echo "compiling $*"
	ps2pdf $< $*.pdf 

all:: ${PAPER_ROOT}.view

outline:: ${OUTLINE}.view

gs:: ${PAPER_ROOT}.psview

print: ${PAPER_ROOT}.ps  ${PAPER_ROOT}.pdf
print_outline: ${OUTLINE}.ps
	lpr ${OUTLINE}.ps

${PAPER_ROOT}.dvi: ${INFILES} ${PAPER_ROOT}.bib ${PICTURES}
	latex ${PAPER_ROOT}
	bibtex ${PAPER_ROOT}
	latex ${PAPER_ROOT}
	latex ${PAPER_ROOT}

${OUTLINE}.dvi: ${OUTLINE}.tex ${OUTLINE}.bib ${PICTURES}
	latex ${OUTLINE}
	bibtex ${OUTLINE}
	latex ${OUTLINE}
	latex ${OUTLINE}
	chmod 664 ${OUTLINE}.blg ${OUTLINE}.bbl ${OUTLINE}.aux ${OUTLINE}.dvi ${OUTLINE}.log

${PAPER_ROOT}.psview: ${PAPER_ROOT}.ps
	${PSVIEWER} ${PAPER_ROOT}.ps

${PAPER_ROOT}.view: ${PAPER_ROOT}.dvi
	xdvi ${PAPER_ROOT}

${OUTLINE}.view: ${OUTLINE}.dvi
	xdvi ${OUTLINE}

clean::
	/bin/rm -f *.aux *.log *.bbl *.blg *.dvi *~



